Entanglement Propagation in Integrable Heisenberg Chains from a New Lens

The exact single-magnon entanglement evolution in Heisenberg chains is obtained using the Quantum Correlation Transfer Function (QCTF) formulation. A dual, i.e., frequency and time-domain, analysis shows that the transient dynamics of individual spins' entanglement is described via a Bessel function of the first kind. Through QCTF, we bypass the evaluation of the full system's state for the purpose of obtaining entanglement. Although it is known that the observable entanglement edge is formed by the arrival of a stream of quasi-particles that travel with the maximum group velocity, we show how the early quasi-particles travel faster than the maximum group velocity of the chain and contribute to entanglement production. Our results can be extended to the multi-magnon regime, therefore opening up the means to better interpret equilibration dynamics and thermodynamics in Heisenberg chains.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
